LEARNT: A Practical Estimator for Cardinality of LIKE Queries with Formal Accuracy Guarantees

We study the problem of cardinality estimation for LIKE queries on string data, focusing on the most common patterns in real workloads: prefix, suffix, and substring queries. We propose LEARNT, a LIKE query Estimator with Accuracy, Robustness, Negligible overhead, Tunability, and Theoretical guarantees. LEARNT formulates estimation as a bucket-classification problem, and upon correct classification, it yields formal bounds on Q-error for the queries with non-empty answer. It employs a memory-efficient bucketed layered-filter architecture with Bloom filters and compact auxiliary tables, together with optimizations that exploit query skew to reduce storage. For the queries that have empty answer, LEARNT incorporates dedicated filter-based and prefix-walk strategies, providing probabilistic guarantees on correct identification. Furthermore, to support arbitrarily long query strings, we extend LEARNT with Markov modeling scheme that composes short-query statistics into estimates for longer queries. A theoretical framework guides parameter selection to minimize storage under accuracy and robustness constraints. Extensive experiments on four real-world datasets show that LEARNT consistently outperforms state-of-the-art methods such as CLIQUE and LPLM, achieving 1.3-1.7x lower mean Q-error, significantly lower tail errors, and up to 70x faster construction with comparable memory usage.

==> algo/greedy_selection.tex <==
\begin{algorithm}[t]
\caption{Greedy Set Cover with Inverted Index and Heap}
\label{alg:greedy_set_cover}
\KwIn{List of subsets $\{S_1, S_2, \dots, S_n\}$ where each $S_i$ is a set of query IDs; maximum iterations $T$}
\KwOut{Selected subset indices $\mathcal{P}$ covering all elements}
\BlankLine
Initialize inverted index: element $\to$ list of subsets containing it\;
Initialize uncovered counts $C[S_i] = |S_i|$ for each $S_i$\;
Insert $( -C[S_i], i )$ into max-heap $H$ for all $i$\;
Initialize covered set $U = \emptyset$ and result set $\mathcal{P} = \emptyset$\;
\For{iteration $= 1$ to $T$}{
    \While{$H$ not empty}{
        Pop $(c, j)$ from $H$\;
        \If{$-c = C[S_j]$}{ break\; }
    }
    \If{$C[S_j] = 0$}{ break\;}
    Add $j$ to $\mathcal{P}$\;
    \For{each element $e \in S_j$}{
        \If{$e \notin U$}{
            Add $e$ to $U$\;
            \For{each $k$ where $S_k$ contains $e$}{
                Decrease $C[S_k]$ by $1$\;
                Push $( -C[S_k], k )$ into $H$\;
            }
        }
    }
    Optionally rebuild heap every $R$ iterations (to remove stale entries)\;
    \If{all elements covered ($|U| = |\mathcal{U}|$)}{ break\; }
}
\Return $\mathcal{P}$
\end{algorithm}

==> figure/model_arch.tex <==
\begin{figure}[t]
    \vspace{-1em}
	\centering
	\includegraphics[width=0.47\textwidth]{ figure/model_design.pdf}
	\vspace{-1em}
	\caption{Proposed Learning-based Framework}
	\label{fg:learning-ov}
	% \vspace{-6mm}
\end{figure}

==> figure/tree_structure.tex <==
\begin{figure}[t]
    \vspace{-1em}
	\centering
	\includegraphics[width=0.40\textwidth]{ figure/tree_structure.pdf}
	\vspace{-1em}
	\caption{Tree Structures}
	\label{fg:tree-ov}
	\vspace{-6mm}
\end{figure}

==> tab/accuracy_basic_author.tex <==


\begin{table}[!ht]
	\small
	% \vspace{-3mm}
	\centering
	\caption{\textsf{Q-error} for Different Estimators on \textit{Author} on Basic Patterns}
	% \vspace{-4mm} 
	\resizebox{0.48\textwidth}{!}{%
		\begin{tabular}{|c|c|c|c|c|c|c|}
			\hline
			\textbf{Pattern Type} & \textbf{Method} & \textbf{Mean} &                \textbf{90th} & \textbf{95th} & \textbf{99th} & \textbf{Max}\\\hline
                \multirow{5}{*}{$S\%$}& PostgreSQL & 9.6&11.0&11.0&11.0&1098.0 \\\cline{2-7}
                & \BF & 1.34\best &1.3 \best &1.54 \best &1.58 \best &1.6\best \\
                \cline{2-7}
                & Astrid & 2.06&1.31\second&4.98&12.15&529.44\\\cline{2-7}
                & E2E & 2.3&1.49&4.54&12.26&1446.39\\\cline{2-7}
                & LPLM & 8.98&3.41&27.69&86.53&7269.58\\\cline{2-7}
                %  & E2E & \textbf{1.69} & \textbf{2.54} & \textbf{2.89} & 6.51 & 1162.63\\\cline{2-7}
                & CLIQUE & 1.7\second &1.35&3.33\second&6.33\second&166.0\second \\\hline
                 \multirow{5}{*}{$\%S$}& PostgreSQL & 9.5&11.0&11.0&11.0&1098.0 \\\cline{2-7}
                & \BF & 1.35\best&1.3\best&1.54\best&1.54\best&1.6\best\\
                \cline{2-7}
                & Astrid & 2.07&1.44\second&4.97&11.22&429.83\\\cline{2-7}
                & E2E & 2.08&1.52&4.11&9.03&589.68\\\cline{2-7}
                & LPLM &4.75&3.42&10.19&22.05&4727.97\\\cline{2-7}
                %  & E2E & \textbf{1.69} & \textbf{2.54} & \textbf{2.89} & 6.51 & 1162.63\\\cline{2-7}
                & CLIQUE & 1.77\second&1.44\second&3.54\second&6.45\second&50.8\second \\\hline
                 \multirow{5}{*}{$\%S\%$}& PostgreSQL & 9.17&11.0&11.0&11.0&1098.0 \\\cline{2-7}
                %  & LBS & 1.41 & 1.41&1.53&1.53&426.93 \\
                % \cline{2-7}
                % & P-LSH & 1.41 & 1.41&1.53&1.53&426.93 \\
                % \cline{2-7}
                & \BF & 1.35\best&1.3\best&1.54\best&1.58\best&1.6\best\\
                \cline{2-7}
                & Astrid & 2.31&1.54&5.25&12.82&3984.62\\\cline{2-7}
                & E2E & 2.37&1.57&4.94&11.73&1278.92 \\\cline{2-7}
                & LPLM & 10.32&4.19&33.89&113.9&9451.88 \\\cline{2-7}
                %  & E2E & \textbf{1.69} & \textbf{2.54} & \textbf{2.89} & 6.51 & 1162.63\\\cline{2-7}
                & CLIQUE & 1.83\second&1.46\second&3.74\second&6.89\second&166.0\second \\\hline
                % \bottomrule
                  \multicolumn{7}{@{}l}{\footnotesize Note: \best\ marks the best (lowest) value, while \second\ marks the second-best.}
                % \multirow{3}{*}{$S\%S\%$}& PostgreSQL & 92.71&8.27&559.18&1188.09&2667.64\\\cline{2-7}
                %  & LPLM &  5.01&2.71&13.46&43.07&1623.95 \\
                % \cline{2-7}
                % & \tocheck{CLIQUE} & 1.89&1.53&3.7&6.65&1927.0 \\
                % \cline{2-7}
                % & \tocheck{Learned} & 2.04&1.69&4.11&7.45&541.64\\\hline
                % \multirow{3}{*}{$S\%S$}& PostgreSQL &26.02&3.67&102.73&401.82&838.27\\\cline{2-7}
                %  & LPLM & 6.83&3.31&20.31&70.21&2290.91 \\
                % \cline{2-7}
                % & \tocheck{CLIQUE} & 1.69&1.46&3.15&5.07&41.0 \\
                % \cline{2-7}
                % & \tocheck{Learned} & 1.91&1.68&3.66&6.23&22.71\\\hline
                % \multirow{3}{*}{$\%S\%S\%$}& PostgreSQL &98.25&8.45&571.45&1279.64&2667.64\\\cline{2-7}
                %  & LPLM & 3.12&2.38&6.68&11.86&690.81 \\
                % \cline{2-7}
                % & \tocheck{CLIQUE} & 1.94&1.58&3.94&7.04&251.57 \\
                % \cline{2-7}
                % & \tocheck{Learned} & 2.06&1.74&4.13&7.57&134.73\\\hline
                % \multirow{3}{*}{$\%S\%S$}& PostgreSQL &121.52&16.45&653.27&1391.09&2667.64\\\cline{2-7}
                %  & LPLM & 3.86&2.83&9.14&20.31&421.12 \\
                % \cline{2-7}
                % & \tocheck{CLIQUE} & 1.86&1.55&3.65&6.32&114.38 \\
                % \cline{2-7}
                % & \tocheck{Learned} & 2.02&1.72&4.03&7.18&100.91\\\hline
		\end{tabular}%
	}
	\label{tab:basic-acc-author}
	% \vspace{-4mm}
\end{table}

==> tab/accuracy_basic_dblp_an.tex <==
\begin{table}[!ht]
	\small
	% \vspace{-3mm}
	\centering
	\caption{\textsf{Q-error} for Different Estimators on \textit{DBLP-AN} on Basic Patterns}
	% \vspace{-4mm} 
	\resizebox{0.48\textwidth}{!}{%
		\begin{tabular}{|c|c|c|c|c|c|c|}
			\hline
			\textbf{Pattern Type} & \textbf{Method} & \textbf{Mean} &                \textbf{90th} & \textbf{95th} & \textbf{99th} & \textbf{Max}\\\hline
                \multirow{5}{*}{$S\%$}& PostgreSQL & 7.99&11.0&11.0&11.0&1355.18 \\\cline{2-7}
                & \BF & 1.35\best&1.3\best&1.54\best&1.58\best&1.6\best \\
                \cline{2-7}
                & Astrid & 2.4&1.67&5.73&14.21&482.96\\\cline{2-7}
                & E2E & 2.57&1.82&5.37&15.26&474.23\\\cline{2-7}
                & LPLM & 8.95&3.11&30.54&102.48&5303.01\\\cline{2-7}
                %  & E2E & \textbf{1.69} & \textbf{2.54} & \textbf{2.89} & 6.51 & 1162.63\\\cline{2-7}
                & CLIQUE & 2.19\second&1.62\second&4.85\second&11.4\second&589.77\second \\\hline
                 \multirow{5}{*}{$\%S$}& PostgreSQL & 7.91&11.0&11.0&11.0&2257.18 \\\cline{2-7}
                & \BF & 1.35\best&1.3\best&1.54\best&1.58\best&1.6\best\\
                \cline{2-7}
                & Astrid & 2.49&1.77&5.69&14.89&1924.61\\\cline{2-7}
                & E2E & 2.44&1.83&5.14&12.62&842.46 \\\cline{2-7}
                & LPLM &  6.25&3.14&11.82&33.73&23830.59 \\\cline{2-7}
                %  & E2E & \textbf{1.69} & \textbf{2.54} & \textbf{2.89} & 6.51 & 1162.63\\\cline{2-7}
                & CLIQUE & 2.23\second&1.75\second&4.82\second&10.84\second&267.64\second \\\hline
                 \multirow{5}{*}{$\%S\%$}& PostgreSQL & 7.74&11.0&11.0&11.0&1547.0 \\\cline{2-7}
                %  & LBS & 1.41 & 1.41&1.53&1.53&426.93 \\
                % \cline{2-7}
                % & P-LSH & 1.41 & 1.41&1.53&1.53&426.93 \\
                % \cline{2-7}
                & \BF & 1.35\best&1.3\best&1.54\best&1.58\best&1.6\best\\
                \cline{2-7}
                & Astrid & 2.05\second & 2.92 & 4.50 & 14.55 & 1768.54\\\cline{2-7}
                & E2E & 2.72&1.88&6.04&17.02&847.46\\\cline{2-7}
                & LPLM & 114.86&4.05&45.79&190.55&17860.03\\\cline{2-7}
                %  & E2E & \textbf{1.69} & \textbf{2.54} & \textbf{2.89} & 6.51 & 1162.63\\\cline{2-7}
                & CLIQUE & 2.3&1.72\second&5.18\second&11.93\second&479.0\second \\\hline
                % \multirow{3}{*}{$S\%S\%$}& PostgreSQL &  101.64&8.34&623.42&1525.07&3463.44\\\cline{2-7}
                %  & LPLM & 6.46&3.03&19.2&64.48&2265.05 \\
                % \cline{2-7}
                % & CLIQUE & 2.27&1.75&4.97&10.75&640.14 \\
                % \cline{2-7}
                % & Learned & 2.36&1.86&5.06&10.5&376.3\\\hline
                % \multirow{3}{*}{$S\%S$}& PostgreSQL &23.8&5.0&95.27&438.58&1501.0 \\\cline{2-7}
                %  & LPLM &10.59&3.77&32.05&128.83&4973.78\\
                % \cline{2-7}
                % & CLIQUE & 2.13&1.79&4.33&8.69&69.06 \\
                % \cline{2-7}
                % & Learned &2.21&1.84&4.55&8.97&75.97\\\hline
                % \multirow{3}{*}{$\%S\%S\%$}& PostgreSQL & 95.99&7.58&592.38&1525.07&3463.44\\\cline{2-7}
                %  & LPLM & 3.68&2.59&8.76&17.66&1357.24\\
                % \cline{2-7}
                % & CLIQUE & 2.32&1.79&5.13&10.97&378.51 \\
                % \cline{2-7}
                % & Learned &2.42&1.9&5.25&10.82&335.81\\\hline
                % \multirow{3}{*}{$\%S\%S$}& PostgreSQL & 132.28&13.62&782.51&1574.49&3463.44\\\cline{2-7}
                %  & LPLM & 5.0&3.05&11.82&33.44&2733.67 \\
                % \cline{2-7}
                % & CLIQUE & 2.27&1.86&4.77&10.05&145.62 \\
                % \cline{2-7}
                % & Learned & 2.34&1.93&4.78&9.7&271.96\\\hline
		\end{tabular}%
	}
	\label{tab:basic-acc-dblp-an}
	% \vspace{-4mm}
\end{table}

==> tab/accuracy_basic_imdb_an.tex <==
\begin{table}[!ht]
	\small
	% \vspace{-3mm}
	\centering
	\caption{\textsf{Q-error} for Different Estimators on \textit{IMDB-AN} on Basic Patterns}
	% \vspace{-4mm} 
	\resizebox{0.48\textwidth}{!}{%
		\begin{tabular}{|c|c|c|c|c|c|c|}
			\hline
			\textbf{Pattern Type} & \textbf{Method} & \textbf{Mean} &                \textbf{90th} & \textbf{95th} & \textbf{99th} & \textbf{Max}\\\hline
                \multirow{5}{*}{$S\%$}& PostgreSQL & 9.81&11.0&11.0&11.0&838.09 \\\cline{2-7}
                & \BF & 1.33\best&1.3&1.54\best&1.54\best&1.6\best \\
                \cline{2-7}
                & Astrid & 1.66&1.0\best&3.48&10.58&1098.55\\\cline{2-7}
                & E2E & 1.74&1.01\second&3.72&10.73&370.95\\\cline{2-7}
                & LPLM & 4.93&2.73&10.88&34.65&10829.71\\\cline{2-7}
                %  & E2E & \textbf{1.69} & \textbf{2.54} & \textbf{2.89} & 6.51 & 1162.63\\\cline{2-7}
                & CLIQUE & 1.5\second&1.07&2.87\second&7.24\second&292.02\second \\\hline
                 \multirow{5}{*}{$\%S$}& PostgreSQL & 9.83&11.0&11.0&11.0&7220.64 \\\cline{2-7}
                & \BF & 1.33\best&1.3&1.54\best&1.54\best&1.6\best\\
                \cline{2-7}
                & Astrid & 1.94&1.01\best&4.08&13.46&1187.26\\\cline{2-7}
                & E2E & 1.99&1.06\second&4.0&12.88&12785.0 \\\cline{2-7}
                & LPLM & 7.57&3.21&15.99&69.68&10798.68\\\cline{2-7}
                %  & E2E & \textbf{1.69} & \textbf{2.54} & \textbf{2.89} & 6.51 & 1162.63\\\cline{2-7}
                & CLIQUE & 1.59\second&1.1&2.87\second&7.82\second&927.21\second \\\hline
                 \multirow{5}{*}{$\%S\%$}& PostgreSQL & 9.5&11.0&11.0&11.0&5213.55 \\\cline{2-7}
                %  & LBS & 1.41 & 1.41&1.53&1.53&426.93 \\
                % \cline{2-7}
                % & P-LSH & 1.41 & 1.41&1.53&1.53&426.93 \\
                % \cline{2-7}
                & \BF & 1.33\best&1.3&1.54\best&1.54\best&1.6\best\\
                \cline{2-7}
                & Astrid & 2.27&1.12\best&4.91&16.03&8367.11\\\cline{2-7}
                & E2E & 2.14&1.16&4.77&16.15&2901.0 \\\cline{2-7}
                & LPLM &  9.93&3.84&25.09&92.56&15360.61\\\cline{2-7}
                %  & E2E & \textbf{1.69} & \textbf{2.54} & \textbf{2.89} & 6.51 & 1162.63\\\cline{2-7}
                & CLIQUE & 1.62\second&1.13\second&3.2\second&7.91\second&557.28\second \\\hline
                % \multirow{3}{*}{$S\%S\%$}& PostgreSQL &  125.04&16.05&716.13&1555.69&2916.33\\\cline{2-7}
                %  & LPLM & 4.25&2.61&10.41&32.98&1103.5\\
                % \cline{2-7}
                % & CLIQUE & 1.47&1.12&2.8&5.58&262.05 \\
                % \cline{2-7}
                % & Learned & 1.64&1.38&2.82&5.93&425.0\\\hline
                % \multirow{3}{*}{$S\%S$}& PostgreSQL &27.22&8.0&111.95&328.82&1852.0 \\\cline{2-7}
                %  & LPLM &  7.77&3.3&21.34&80.47&4714.56\\
                % \cline{2-7}
                % & CLIQUE & 1.26&1.07&2.08&3.36&41.47 \\
                % \cline{2-7}
                % & Learned & 1.41&1.29&2.2&3.69&31.89\\\hline
                % \multirow{3}{*}{$\%S\%S\%$}& PostgreSQL & 111.18&13.43&636.56&1467.85&2916.33\\\cline{2-7}
                %  & LPLM & 3.25&2.43&6.47&14.78&784.42 \\
                % \cline{2-7}
                % & CLIQUE & 1.58&1.17&3.1&6.63&296.18 \\
                % \cline{2-7}
                % & Learned & 1.8&1.45&3.37&7.21&356.48\\\hline
                % \multirow{3}{*}{$\%S\%S$}& PostgreSQL & 82.47&7.86&459.18&1264.2&2916.33\\\cline{2-7}
                %  & LPLM & 5.04&2.95&12.01&39.65&2705.74 \\
                % \cline{2-7}
                % & CLIQUE & 1.52&1.16&2.8&5.74&569.93 \\
                % \cline{2-7}
                % & Learned & 1.7&1.4&2.96&5.99&406.75\\\hline
		\end{tabular}%
	}
	\label{tab:basic-acc-imdb-an}
	% \vspace{-4mm}
\end{table}

==> tab/accuracy_basic_imdb_mt.tex <==
\begin{table}[!ht]
	\small
	% \vspace{-3mm}
	\centering
	\caption{\textsf{Q-error} for Different Estimators on \textit{IMDB-MT} on Basic Patterns}
	% \vspace{-4mm} 
	\resizebox{0.48\textwidth}{!}{%
		\begin{tabular}{|c|c|c|c|c|c|c|}
			\hline
			\textbf{Pattern Type} & \textbf{Method} & \textbf{Mean} &                \textbf{90th} & \textbf{95th} & \textbf{99th} & \textbf{Max}\\\hline
                \multirow{5}{*}{$S\%$}& PostgreSQL & 9.36&11.0&11.0&11.0&1098.0 \\\cline{2-7}
                & \BF & 1.33\best&1.3&1.54\best&1.54\best&1.6\best \\
                \cline{2-7}
                & Astrid & 1.77 & 2.44 & 3.87 & 11.99 & 618.67\\\cline{2-7}
                & E2E & 1.99&1.1\best&4.32&12.43&4727.97 \\\cline{2-7}
                & LPLM & 6.55&2.21&16.83&65.66&28987.37\\\cline{2-7}
                %  & E2E & \textbf{1.69} & \textbf{2.54} & \textbf{2.89} & 6.51 & 1162.63\\\cline{2-7}
                & CLIQUE & 1.66\second&1.23\second&3.49\second&8.29\second&215.5\second \\\hline
                 \multirow{5}{*}{$\%S$}& PostgreSQL & 9.46&11.0&11.0&11.0&2226.09 \\\cline{2-7}
                & \BF & 1.33\best&1.3&1.54\best&1.54\best&1.6\best\\
                \cline{2-7}
                % & Astrid & 1.55\second & 1.94 & 2.76\second & 8.65 & 2485.51\\\cline{2-7}
                & Astrid & 1.55\second & 1.94 & 2.76\second & 8.65 & 2485.51\\\cline{2-7}
                & E2E & 1.95&1.12\best&4.25&11.0&1147.66\\\cline{2-7}
                & LPLM & 11.97&3.0&15.68&83.22&87207.32\\\cline{2-7}
                %  & E2E & \textbf{1.69} & \textbf{2.54} & \textbf{2.89} & 6.51 & 1162.63\\\cline{2-7}
                & CLIQUE & 1.62&1.2\second&3.43&8.0\second&356.34\second \\\hline
                 \multirow{5}{*}{$\%S\%$}& PostgreSQL & 9.33&11.0&11.0&11.0&7752.73 \\\cline{2-7}
                %  & LBS & 1.41 & 1.41&1.53&1.53&426.93 \\
                % \cline{2-7}
                % & P-LSH & 1.41 & 1.41&1.53&1.53&426.93 \\
                % \cline{2-7}
                & \BF &1.33\best&1.3&1.54\best&1.54\best&1.6\best\\
                \cline{2-7}
                & Astrid & - & - & - & - & -\\\cline{2-7}
                & E2E & 2.27&1.27\second&4.81&14.39&3961.14 \\\cline{2-7}
                & LPLM & 18.36&3.88&51.58&220.79&45274.68 \\\cline{2-7}
                %  & E2E & \textbf{1.69} & \textbf{2.54} & \textbf{2.89} & 6.51 & 1162.63\\\cline{2-7}
                & CLIQUE & 1.7\second&1.24\best&3.55\second&8.81\second&908.69\second \\\hline
                % \multirow{3}{*}{$S\%S\%$}& PostgreSQL &  125.29&11.42&762.81&1738.64&3700.89\\\cline{2-7}
                %  & LPLM &6.2&2.2&17.02&66.72&13058.1 \\
                % \cline{2-7}
                % & CLIQUE & 1.51&1.19&2.85&6.0&289.62 \\
                % \cline{2-7}
                % & Learned &  1.64&1.35&3.01&6.45&296.3\\\hline
                % \multirow{3}{*}{$S\%S$}& PostgreSQL &20.33&5.11&104.39&274.58&1202.33 \\\cline{2-7}
                %  & LPLM & 13.15&3.2&42.58&170.09&17014.77 \\
                % \cline{2-7}
                % & CLIQUE & 1.35&1.11&2.42&4.62&80.0 \\
                % \cline{2-7}
                % & Learned & 1.44&1.23&2.46&4.93&84.19\\\hline
                % \multirow{3}{*}{$\%S\%S\%$}& PostgreSQL & 91.46&8.03&549.08&1491.14&3700.89\\\cline{2-7}
                %  & LPLM & 3.53&1.87&6.88&24.54&10982.28 \\
                % \cline{2-7}
                % & CLIQUE & 1.53&1.19&2.93&6.03&136.75 \\
                % \cline{2-7}
                % & Learned & 1.69&1.42&3.09&6.31&112.2\\\hline
                % \multirow{3}{*}{$\%S\%S$}& PostgreSQL & 127.27&11.58&764.92&1738.64&3700.89\\\cline{2-7}
                %  & LPLM & 6.99&2.48&16.19&70.34&20404.41 \\
                % \cline{2-7}
                % & CLIQUE & 1.47&1.15&2.79&5.72&121.35 \\
                % \cline{2-7}
                % & Learned & 1.61&1.35&2.89&6.03&143.91\\\hline
                % \multicolumn{7}{@{}l}{ }
		\end{tabular}%
	}
	\label{tab:basic-acc-imdb-mt}
	% \vspace{-4mm}
\end{table}

==> tab/basic_diff_range.tex <==
\begin{table}[!ht]
	\small
	% \vspace{-3mm}
	\centering
	\caption{Mean Q-error of Each Method on \textit{Actor} in Different Cardinality Ranges}
	% \vspace{-4mm} 
	\resizebox{0.48\textwidth}{!}{%
		\begin{tabular}{|c|c|c|c|c|c|c|c|}
			\hline
			\textbf{Pattern Type} & \textbf{Method} & \textbf{[1-2]} &                \textbf{[3-7]} & \textbf{[8-20]} & \textbf{[21-53]} & \textbf{[54-138]} & \textbf{[139,)}\\\hline
                \multirow{4}{*}{$S\%$}& PostgreSQL & 53.48&15.26&6.1&2.87&2.23&7.24\\\cline{2-8}
                & BF & 1.33&1.36&1.31&1.29&1.3&1.34 \\
                \cline{2-8}
                & Astrid & 1.25&2.94&6.92&14.79&28.23&51.51\\\cline{2-8}
                & LPLM & 3.32&4.36&4.06&3.03&2.2&1.34\\\hline
                %  & E2E & \textbf{1.69} & \textbf{2.54} & \textbf{2.89} & 6.51 & 1162.63\\\cline{2-7}
                % & FACE & 1.81 & 2.71 & 3.50 & \textbf{6.00} & 672.48 \\\hline
                 \multirow{4}{*}{$\%S$}& PostgreSQL & 52.49&14.82&5.38&2.41&2.08&9.66\\\cline{2-8}
                & BF & 1.33&1.35&1.31&1.29&1.28&1.33\\
                \cline{2-8}
                & Astrid & 1.14&3.53&9.02&21.27&44.25&141.2\\\cline{2-8}
                & LPLM &  & &  &  & &\\\hline
                %  & E2E & \textbf{1.69} & \textbf{2.54} & \textbf{2.89} & 6.51 & 1162.63\\\cline{2-7}
                % & FACE & 1.81 & 2.71 & 3.50 & \textbf{6.00} & 672.48 \\\hline
                 \multirow{4}{*}{$\%S\%$}& PostgreSQL & 52.58&15.65&6.02&2.88&2.61&9.19\\\cline{2-8}
                %  & LBS & 1.41 & 1.41&1.53&1.53&426.93 \\
                % \cline{2-7}
                % & P-LSH & 1.41 & 1.41&1.53&1.53&426.93 \\
                % \cline{2-7}
                & BF & 1.33&1.35&1.31&1.29&1.28&1.35\\
                \cline{2-8}
                & Astrid & 1.34&2.88&6.55&13.59&26.89&78.02\\\cline{2-8}
                & LPLM &  &  &  &  & &\\\hline %\cline{2-7}
                %  & E2E & \textbf{1.69} & \textbf{2.54} & \textbf{2.89} & 6.51 & 1162.63\\\cline{2-7}
                % & FACE & 1.81 & 2.71 & 3.50 & \textbf{6.00} & 672.48 \\\hline
		\end{tabular}%
	}
	\label{tab:qe-actor-basic-diffrange}
	% \vspace{-4mm}
\end{table}

==> tab/overall_est.tex <==
\begin{table*}[ht]
\centering
\caption{Q-error for Different Estimators on Valid Queries}
\label{tab:qerror_basic_patterns}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|}
% \toprule
\hline
\multirow{2}{*}{Query} & \multirow{2}{*}{Method}
  & \multicolumn{5}{c|}{Author} 
  & \multicolumn{5}{c|}{IMDB-AN} \\\cline{3-12}
 & & Mean & 90th & 95th & 99th & Max 
     & Mean & 90th & 95th & 99th & Max \\\hline
% \midrule
\multirow{6}{*}{S\%}
  & PostgreSQL      &  9.6   & 11.0 & 11.0 & 11.0  & 1098.0   
                   &  9.81  & 11.0 & 11.0 & 11.0  & 838.09   \\
  & \BF{}    &  1.38\best&1.41\second&1.41\best&1.46\best&1.5\best 
                   &  1.4\best&1.41&1.41\best&1.41\best&1.5\best  \\
 
  & E2E             &  2.30  & 1.49  & 4.54   & 12.26 & 1446.39 
                   &  1.74   & 1.01\second & 3.72  & 10.73 & 370.95  \\
                    & Astrid          &  1.94&1.24&4.76&10.68&412.31  
                   &  1.61&1.0&3.25&9.5&876.22 \\
  & LPLM            &  8.98  & 3.41  & 27.69  & 86.53 & 7269.58 
                   &  4.93   & 2.73  & 10.88 & 34.65 & 10829.71\\
  & CLIQUE          &  1.7\second & 1.35  & 3.33\second & 6.33\second & 166.0\second 
                   &  1.5\second  & 1.07  & 2.87\second & 7.24\second & 292.02  \\
\hline
\multirow{6}{*}{\%S}
  & PostgreSQL      &  9.5   & 11.0 & 11.0 & 11.0  & 1098.0   
                   &  9.83&11.0&11.0&11.0&7220.64  \\
  & \BF{}    &  1.38\best&1.41\best&1.41\best&1.46\best&1.5\best  
                   &  1.4\best&1.41&1.41\best&1.46\best&1.5\best  \\
 
  & E2E             &  2.08  & 1.52  & 4.11   & 9.03  & 589.68  
                   &  1.99   & 1.06\second     & 4.00  & 12.88 & 12785.0 \\
 & Astrid          &  2.63&1.3&7.0&17.49&3418.58  
                   &  2.32&1.0&4.63&19.98&4606.3 \\
  & LPLM            &  4.75  & 3.42  & 10.19  & 22.05 & 4727.97 
                   &  7.57&3.21&15.99&69.68&10798.68\\
  & CLIQUE          &  1.77\second&1.44\second&3.54\second&6.45\second&50.8\second  
                   &  1.59\second&1.1&2.87\second&7.82\second&927.21\second \\
\hline
\multirow{9}{*}{\%S\%}
  & PostgreSQL      &  9.17  & 11.0 & 11.0 & 11.0  & 1098.0   
                   &  9.50  & 11.0 & 11.0 & 11.0  & 5213.55  \\
  & MO             & 2.88&1.0\best&5.85&11.01&16056.0
                    & 1.51&1.0\best&3.0\second&6.0\second&19600.0  \\
  & LBS             & 2.15&1.0\best&7.0&13.0&39.4\second
                    & 1.52&1.0\best&4.0&9.0&117.07  \\
    
  & \BF{}    &  1.38\best&1.41\second&1.41\best&1.46\best&1.5\best  
                   &  1.4\best&1.41&1.41\best&1.46\best&1.5\best  \\
 
  & E2E             &  2.37  & 1.57  & 4.94   & 11.73 & 1278.92 
                   &  2.14&1.16&4.77&16.15&2901.0 \\[-0.5ex]
 & Astrid          &  2.92&1.42&7.51&20.46&6879.51 
                   &  2.83&1.0&5.74&24.89&8016.84 \\[-0.5ex]
  & LPLM            & 10.32  & 4.19  & 33.89  & 113.9 & 9451.88 
                   & 9.93&3.84&25.09&92.56&15360.61 \\
  & CLIQUE          &  1.83\second&1.46&3.74\second&6.89\second&166.0  
                   &  1.62&1.13&3.2&7.91&557.28 \\
  & SSCard        & 2.02&1.0\best&6.0&12.0&59.0
                    & 1.45\second&1.0\best&3.0\second&7.0&72.0\second  \\
\hline\hline
\multirow{2}{*}{Query} & \multirow{2}{*}{Method}
  & \multicolumn{5}{c|}{DBLP-AN} 
  & \multicolumn{5}{c|}{IMDB-MT} \\\cline{3-12}
 & & Mean & 90th & 95th & 99th & Max 
     & Mean & 90th & 95th & 99th & Max \\
\hline
\multirow{6}{*}{S\%}
  & PostgreSQL      &  7.99  & 11.0  & 11.0  & 11.0   & 1355.18  
                   &  9.36  & 11.0  & 11.0  & 11.0   & 1098.0   \\
  
  & \BF{}    &  1.37\best&1.41\best&1.41\best&1.46\best&1.5\best  
                   &  1.39\best&1.41&1.41\best&1.46\best&1.5\best  \\
  
  & E2E             &  2.57  & 1.82  & 5.37   & 15.26 & 474.23  
                   &  1.99  & 1.10\best & 4.32   & 12.43 & 4727.97  \\
   & Astrid          &  2.32&1.67&5.48&12.76&768.65  
                   &  1.78&1.03&4.18&11.78&211.02   \\
  & LPLM            &  8.95  & 3.11  & 30.54  & 102.48& 5303.01 
                   &  6.55  & 2.21  & 16.83  & 65.66 & 28987.37 \\
  & CLIQUE          &  2.19\second&1.62\second&4.85\second&11.4\second&589.77\second  
                   &  1.66\second&1.23\second&3.49\second&8.29\second&215.5\second \\
\hline
\multirow{6}{*}{\%S}
  & PostgreSQL      &  7.91  & 11.0  & 11.0  & 11.0   & 2257.18  
                   &  9.46  & 11.0  & 11.0  & 11.0   & 2226.09  \\
  & \BF{}    &  1.37\best&1.41\best&1.41\best&1.46\best&1.5\best  
                   &  1.39\best&1.41&1.41\best&1.46\best&1.5\best  \\
  
  & E2E             &  2.44  & 1.83  & 5.14   & 12.62 & 842.46  
                   &  1.95  & 1.12$^*$ & 4.25   & 11.00 & 1147.66  \\
& Astrid          &  3.02&1.62&8.01&22.49&2833.54 
                   &  2.07&1.01&4.99&16.88&1731.33  \\
  & LPLM            &  6.25  & 3.14  & 11.82  & 33.73 & 23830.59
                   & 11.97  & 3.00  & 15.68  & 83.22 & 87207.32 \\
  & CLIQUE          &  2.23\second&1.75\second&4.82\second&10.84\second&267.64\second  
                   &  1.62&1.2\second&3.43&8.0\second&356.34\second \\
\hline
\multirow{9}{*}{\%S\%}
  & PostgreSQL      &  7.74  & 11.0  & 11.0  & 11.0\second  & 1547.0   
                   &  9.33  & 11.0  & 11.0  & 11.0   & 7752.73  \\
  & MO             & 2.33&1.02\second&7.0&14.0&1321.31
                    & 1.5\second&1.0\best&3.0\second&5.6\second&4542.0  \\
    & LBS             & 2.47&1.0\best&8.0&15.26&277.15
                    & 1.62&1.0\best&4.0&10.0&90.91  \\
   
  & \BF{}    &  1.37\best&1.41&1.41\best&1.46\best&1.5\best  
                   &  1.39\best&1.41&1.41\best&1.46\best&1.5\best  \\
  
  & E2E             &  2.72  & 1.88  & 6.04   & 17.02 & 847.46  
                   &  2.27  & 1.27 & 4.81   & 14.39 & 3961.14  \\
& Astrid          &  3.37&1.68&8.91&27.9&6385.91 
                   &   2.68&1.01&5.98&23.96&6345.04      \\
  & LPLM            &114.86  & 4.05  & 45.79  & 190.55&17860.03
                   & 18.36  & 3.88  & 51.58  & 220.79&45274.68 \\
  & CLIQUE          &  2.3&1.72&5.18&11.93&479.0  
                   &  1.7&1.24\second&3.55&8.81&908.69 \\
     & SSCard        & 2.41&1.0\best&7.0&16.0&82.0\second
                    & 1.58&1.0\best&4.0&9.0&71.0\second  \\\hline
                   \multicolumn{12}{@{}l}{\footnotesize Note: \best\ marks the best (lowest) value, while \second\ marks the second-best.}
\end{tabular}\label{tab:basic-valid-acc}
\end{table*}
